RDRN: Recursively Defined Residual Network for Image Super-Resolution

Deep convolutional neural networks (CNNs) have obtained remarkable performance in single image super-resolution (SISR). However, very deep networks can suffer from training difficulty and hardly achieve further performance gain. There are two main trends to solve that problem: improving the network architecture for better propagation of features through large number of layers and designing an attention mechanism for selecting most informative features. Recent SISR solutions propose advanced attention and self-attention mechanisms. However, constructing a network to use an attention block in the most efficient way is a challenging problem. To address this issue, we propose a general recursively defined residual block (RDRB) for better feature extraction and propagation through network layers. Based on RDRB we designed recursively defined residual network (RDRN), a novel network architecture which utilizes attention blocks efficiently. Extensive experiments show that the proposed model achieves state-of-the-art results on several popular super-resolution benchmarks and outperforms previous methods by up to 0.43 dB.

==> bi_visual.tex <==

\begin{figure*}[t]
	%\newlength-4mm
	%\setlength{-4mm}{-0.4cm}
	\scriptsize
	\centering
	\begin{tabular}{cc}
		
		% % one row
		\hspace{-0.4cm}
		\begin{adjustbox}{valign=t}
			\begin{tabular}{c}
				\includegraphics[width=0.22\textwidth]{images/visual/BI/Urban100/x2/005/Urban100_xx2_5_50_100_170_320_hr-orig-rect.png}
				\\
				Urban100: img\_005 ($\times$2)
			\end{tabular}
		\end{adjustbox}
		\hspace{-0.46cm}
		\begin{adjustbox}{valign=t}
			\begin{tabular}{cccccc}
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/005/Urban100_xx2_5_50_100_170_320_hr-crop.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/005/Urban100_xx2_5_50_100_170_320_bicubic.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/005/Urban100_xx2_5_50_100_170_320_RDN.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/005/Urban100_xx2_5_50_100_170_320_RCAN.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/005/Urban100_xx2_5_50_100_170_320_SAN.png} \hspace{-4mm}
				\\
				HR \hspace{-4mm} &
				Bicubic \hspace{-4mm} &
				RDN~\cite{zhang2018residual} \hspace{-4mm} &
				RCAN~\cite{zhang2018image} \hspace{-4mm} &
				SAN~\cite{dai2019second} \hspace{-4mm}
				\\
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/005/Urban100_xx2_5_50_100_170_320_RFANet.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/005/Urban100_xx2_5_50_100_170_320_DRLN.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/005/Urban100_xx2_5_50_100_170_320_HAN.png} \hspace{-4mm} &		\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/005/Urban100_xx2_5_50_100_170_320_SwinIR.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/005/Urban100_xx2_5_50_100_170_320_XXXN.png} \hspace{-4mm} 
				\\ 
				RFANet~\cite{RFANet}  \hspace{-4mm} &
				DRLN ~\cite{anwar2019drln}  \hspace{-4mm} &
				HAN ~\cite{HAN}  \hspace{-4mm} &
				SwinIR ~\cite{swinir}  \hspace{-4mm} &
				\model (ours) \hspace{-4mm}
				\\
			\end{tabular}
		\end{adjustbox}
		\vspace{1mm}
		\\
		
		% % one row
		\hspace{-0.4cm}
		\begin{adjustbox}{valign=t}
			\begin{tabular}{c}
				\includegraphics[width=0.22\textwidth]{images/visual/BI/Urban100/x2/099/Urban100_xx2_99_590_640_860_1010_hr-orig-rect.png}
				\\
				Urban100: img\_100 ($\times$2)
			\end{tabular}
		\end{adjustbox}
		\hspace{-0.46cm}
		\begin{adjustbox}{valign=t}
			\begin{tabular}{cccccc}
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/099/Urban100_xx2_99_590_640_860_1010_hr-crop.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/099/Urban100_xx2_99_590_640_860_1010_bicubic.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/099/Urban100_xx2_99_590_640_860_1010_RDN.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/099/Urban100_xx2_99_590_640_860_1010_RCAN.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/099/Urban100_xx2_99_590_640_860_1010_SAN.png} \hspace{-4mm}
				\\
				HR \hspace{-4mm} &
				Bicubic \hspace{-4mm} &
				RDN~\cite{zhang2018residual} \hspace{-4mm} &
				RCAN~\cite{zhang2018image} \hspace{-4mm} &
				SAN~\cite{dai2019second} \hspace{-4mm}
				\\
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/099/Urban100_xx2_99_590_640_860_1010_RFANet.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/099/Urban100_xx2_99_590_640_860_1010_DRLN.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/099/Urban100_xx2_99_590_640_860_1010_HAN.png} \hspace{-4mm} &		\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/099/Urban100_xx2_99_590_640_860_1010_SwinIR.png} \hspace{-4mm} &
				\includegraphics[width=0.173\textwidth]{images/visual/BI/Urban100/x2/099/Urban100_xx2_99_590_640_860_1010_XXXN.png} \hspace{-4mm} 
				\\ 
				RFANet~\cite{RFANet}  \hspace{-4mm} &
				DRLN ~\cite{anwar2019drln}  \hspace{-4mm} &
				HAN ~\cite{HAN}  \hspace{-4mm} &
				SwinIR ~\cite{swinir}  \hspace{-4mm} &
				\model (ours) \hspace{-4mm}
				\\
			\end{tabular}
		\end{adjustbox}
		\vspace{1mm}
		\\
		
	\end{tabular}
	\caption{Visual comparison for $2\times$ SR with BI model on Urban100 dataset.  
	}
	\label{fig:visual_result_SRBIX2}
	%\vspace{-5mm}
\end{figure*}

==> complementary.tex <==
\begin{figure*}[t]
%\newlength-4mm
%\setlength{-4mm}{-0.4cm}
\scriptsize
\centering
\begin{tabular}{cc}
% % one row
\hspace{-0.4cm}
\begin{adjustbox}{valign=t}
\begin{tabular}{c}
\includegraphics[width=0.197\textwidth]{figs/visual/large/Resize_ComL_img_044_HR_x4.png}
\\
Urban100: img\_044 ($\times$4)
\end{tabular}
\end{adjustbox}
\hspace{-0.46cm}
\begin{adjustbox}{valign=t}
\begin{tabular}{cccccc}
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_044_HR_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_044_Bicubic_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_044_EDSR_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_044_RDN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_044_RCA_x4.png} \hspace{-4mm} 
\\
HQ \hspace{-4mm} &
Bicubic \hspace{-4mm} &
EDSR~\cite{lim2017enhanced} \hspace{-4mm} &
RDN~\cite{zhang2018residual} \hspace{-4mm} &
RCAN~\cite{zhang2018image} \hspace{-4mm}
\\
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_044_SRFBN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_044_IGNN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_044_CSNLN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_044_RFANet_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_044_RCANit_x4.png} \hspace{-4mm}  
\\ 
SRFBN~\cite{li2019feedback} \hspace{-4mm} &
IGNN~\cite{zhou2020cross} \hspace{-4mm} &
CSNLN~\cite{mei2020image} \hspace{-4mm} &
RFANet~\cite{liu2020residual}  \hspace{-4mm} &
RCAN-it (ours) \hspace{-4mm}
\\
\end{tabular}
\end{adjustbox}
\vspace{1mm}
\\
% % one row
\hspace{-0.4cm}
\begin{adjustbox}{valign=t}
\begin{tabular}{c}
\includegraphics[width=0.197\textwidth]{figs/visual/large/Resize_ComL_img_067_HR_x4.png}
\\
Urban100: img\_067 ($\times$4)
\end{tabular}
\end{adjustbox}
\hspace{-0.46cm}
\begin{adjustbox}{valign=t}
\begin{tabular}{cccccc}
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_067_HR_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_067_Bicubic_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_067_EDSR_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_067_RDN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_067_RCA_x4.png} \hspace{-4mm} 
\\
HQ \hspace{-4mm} &
Bicubic \hspace{-4mm} &
EDSR~\cite{lim2017enhanced} \hspace{-4mm} &
RDN~\cite{zhang2018residual} \hspace{-4mm} &
RCAN~\cite{zhang2018image} \hspace{-4mm}
\\
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_067_SRFBN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_067_IGNN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_067_CSNLN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_067_RFANet_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_067_RCANit_x4.png} \hspace{-4mm}  
\\ 
SRFBN~\cite{li2019feedback} \hspace{-4mm} &
IGNN~\cite{zhou2020cross} \hspace{-4mm} &
CSNLN~\cite{mei2020image} \hspace{-4mm} &
RFANet~\cite{liu2020residual}  \hspace{-4mm} &
RCAN-it (ours) \hspace{-4mm}
\\
\end{tabular}
\end{adjustbox}
\vspace{1mm}
\\
% % one row
\hspace{-0.4cm}
\begin{adjustbox}{valign=t}
\begin{tabular}{c}
\includegraphics[width=0.197\textwidth]{figs/visual/large/Resize_ComL_img_078_HR_x4.png}
\\
Urban100: img\_078 ($\times$4)
\end{tabular}
\end{adjustbox}
\hspace{-0.46cm}
\begin{adjustbox}{valign=t}
\begin{tabular}{cccccc}
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_078_HR_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_078_Bicubic_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_078_EDSR_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_078_RDN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_078_RCA_x4.png} \hspace{-4mm} 
\\
HQ \hspace{-4mm} &
Bicubic \hspace{-4mm} &
EDSR~\cite{lim2017enhanced} \hspace{-4mm} &
RDN~\cite{zhang2018residual} \hspace{-4mm} &
RCAN~\cite{zhang2018image} \hspace{-4mm}
\\
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_078_SRFBN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_078_IGNN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_078_CSNLN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_078_RFANet_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_078_RCANit_x4.png} \hspace{-4mm}  
\\ 
SRFBN~\cite{li2019feedback} \hspace{-4mm} &
IGNN~\cite{zhou2020cross} \hspace{-4mm} &
CSNLN~\cite{mei2020image} \hspace{-4mm} &
RFANet~\cite{liu2020residual}  \hspace{-4mm} &
RCAN-it (ours) \hspace{-4mm}
\\
\end{tabular}
\end{adjustbox}
\vspace{1mm}
\\
% % one row
\hspace{-0.45cm}
\begin{adjustbox}{valign=t}
\begin{tabular}{c}
\includegraphics[width=0.197\textwidth]{figs/visual/large/Resize_ComL_img_092_HR_x4.png}
\\
Urban100: img\_092 ($\times$4)
\end{tabular}
\end{adjustbox}
\hspace{-0.46cm}
\begin{adjustbox}{valign=t}
\begin{tabular}{cccccc}
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_092_HR_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_092_Bicubic_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_092_EDSR_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_092_RDN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_092_RCA_x4.png} \hspace{-4mm} 
\\
HQ \hspace{-4mm} &
Bicubic \hspace{-4mm} &
EDSR~\cite{lim2017enhanced} \hspace{-4mm} &
RDN~\cite{zhang2018residual} \hspace{-4mm} &
RCAN~\cite{zhang2018image} \hspace{-4mm}
\\
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_092_SRFBN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_092_IGNN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_092_CSNLN_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/ComS_img_092_RFANet_x4.png} \hspace{-4mm} &
\includegraphics[width=0.138\textwidth]{figs/visual/large/Urban100_x4_91_179_230_480_581_ours_plus_ours.png} \hspace{-4mm}  
\\ 
SRFBN~\cite{li2019feedback} \hspace{-4mm} &
IGNN~\cite{zhou2020cross} \hspace{-4mm} &
CSNLN~\cite{mei2020image} \hspace{-4mm} &
RFANet~\cite{liu2020residual}  \hspace{-4mm} &
\model (ours) \hspace{-4mm}
\\
\end{tabular}
\end{adjustbox}

\end{tabular}
\caption{Visual comparison ($\times$4) with large SR networks on the Urban100~\cite{huang2015single} dataset. Our simply improved RCAN-it can better reconstruct high-frequency details than RCAN~\cite{zhang2018image} and also compare favorably with previous state-of-the-art approaches. 
}
\label{fig:rcanit_visual_result_SRBIX4_large}
%\vspace{-5mm}
\end{figure*}

==> experiments_bi_.tex <==

We compare the proposed algorithm with the following 11 state-of-the-art methods: SRCNN~\cite{dong2014learning}, RDN~\cite{zhang2018residual}, RCAN~\cite{zhang2018image}, SAN~\cite{dai2019second}, NLSN \cite{NLSN}, DRLN \cite{anwar2019drln}, HAN \cite{HAN}, RFANet\cite{RFANet}, CRAN~\cite{CRAN}, SwinIR~\cite{swinir} and NLSN*~\cite{adadm}.
%We also provide more comparisons in supplementary material.
All results we take from the original papers.
Following~\cite{lim2017enhanced,dai2019second,zhang2018image,HAN,swinir},  we provide self-ensemble model and denote it as \model+.


\textbf{Quantitative results.} Table \ref{table-BI} shows the comparison for $\times 2$, $ \times 3$, $\times 4$ SR quantitative results. Compared to the existing methods, our \model{} performs best on all the scales of reconstructed test datasets. Even without self-ensemble, our \model{} outperforms other compared models for upscale factor  $2\times$ and $3 \times$. For $4 \times$ SR our model achieves best PSNR values, however, SSIM score of competitors on several dataset is higher.
Effect of the proposed method is more significant for lower upscale factor. It can be explained by \blockname{} design. Shallow features are propagated for all levels of \blockname{} using long skip connections from input. For lower upscale factor shallow features contain more important information as less information will be missed comparing with higher upscale factors.

\textbf{Visual results.} We show visual comparisons of various methods on Urban100 dataset for $\times 2$ SR in Figure \ref{fig:visual_result_SRBIX4}. Our model obtains better visual quality and recovers more detailed image. Most compared methods recover grid textures of buildings with  blurring artifacts, however \model{} can produces sharper images. The proposed method can maintain a regular structure in difficult cases where previous approaches have failed. To further illustrate the analyses above, we found such cases for $\times 2$ SR and show them in Figure \ref{fig:visual_result_SRBIX2}. The recovered details are more faithful to the ground truth.



==> related_works.tex <==
The computer vision community prospered in past decades riding the wave of deep learning, and the most popular deep neural networks are often built upon basic blocks, in which a series of convolutional layers are stacked sequentially to capture local information within intermediate features. However, the limited receptive field of small convolutional kernels makes it difficult to obtain global information, withholding the networks of high performance on challenging tasks such as classification, detection, and segmentation. Thus, many researchers start to dig deeper into the self-attention based transformers which have the ability to capture long-range information. Here we briefly review the conventional CNNs and recently proposed vision transformers.

\textbf{Convolutional neural networks}.
The first standard CNN was proposed by Yann ~\cite{lenet} for handwritten character recognition, and the past decades have witnessed that many powerful networks~\cite{alexnet,googlenet,vggnet,resnet,densenet} achieved unprecedented success on large scale image classification task~\cite{imagenet}. AlexNet~\cite{alexnet} and VGGNet~\cite{vggnet} showed that a deep neural network composed of convolutional layers and pooling layers can obtain adequate results in recognition. GoogleNet~\cite{googlenet} and InceptionNet~\cite{inceptionv3} demonstrated the effectiveness of multiple paths within a basic block. ResNet~\cite{resnet} showed better generalization by adding shortcut connections every two layers to the base network. To alleviate the limited receptive fields in prior research, some researches~\cite{wang2017residual,cbam,senet,genet,bam,sasa} incorporated attention mechanisms as an operator for adaptation between modalities. Wang \etal~\cite{wang2017residual} proposed to stack attention modules sequentially between the intermediate stages of deep residual networks. SENet~\cite{senet} and GENet~\cite{genet} adaptively recalibrated
channel-wise feature responses by modelling interdependencies between channels. NLNet~\cite{nlnet} incorporated the self-attention mechanism into neural networks, providing pairwise interactions across all spatial positions to augment the long-range dependencies. In addition to above architectural advances, there has also been works~\cite{squeezenet,shufflenetv2,ghostnet} on improving over-parameterized deep neural networks by trading accuracy for efficiency. MobileNets~\cite{mobilenetv2,mobilenetv3} and EfficientNets~\cite{efficientnet} leveraged neural architecture search (NAS) to design efficient mobile-size network and achieved new state-of-the-art results.

\textbf{Convolutional neural networks with Attention}.

\textbf{Vision transformers.}
Since transformers achieved remarkable success in natural language processing (NLP)~\cite{attention,bert}, many attempts~\cite{vit,deit,t2t,pvt,cvt,cpvt,tnt,ceit,swin} have been made to introduce transformer-like architectures to vision tasks. The pioneering work ViT~\cite{vit} directly applied the transformer architecture inherited from NLP to image classification with image patches as input. While ViT required a large private labelled image dataset JFT-300M~\cite{jft} to achieve promising result, DeiT~\cite{deit} introduced a new training paradigm to extend ViT to a data-efficient vision transformer directly trained on ImageNet-1K. T2T-ViT~\cite{t2t} proposed a T2T transformation to embed visual tokens by recursively aggregating neighboring tokens into one token. TNT~\cite{t2t} proposed to model both patch-level and pixel-level representation by the inner and outer transformer block, respectively. PVT~\cite{pvt} introduced the pyramid structure into ViT, which can generate multi-scale feature maps for various pixel-level dense prediction tasks. CPVT~\cite{cpvt} and CvT~\cite{cvt} are the most related to our work which leverage a convolutional projection into conventional transformer block, but we carefully investigate how to maximize the advantage of utilizing both CNNs and transformers by studying the different components including shortcut and normalization functions and successfully obtain a more superior result. Besides, transformers are also used to solve other vision tasks such as object detection~\cite{detr,deformable-detr}, semantic segmentation~\cite{setr}, image retrieval~\cite{retrieval}, and low-level vision task~\cite{ipt}.

Although there are many works successfully applying transformers for vision tasks, they have not shown satisfactory results compared to conventional CNNs, which are still the primary architectures for vision applications. Transformers are especially good at modelling long-range dependencies necessary for downstream vision tasks. However, locality should also be maintained for visual perception. In this paper, we demonstrate the potential of combining the transformer based network together with convolutional layer, the overall architecture follows the elaborated prior convolutional neural networks such as ResNet~\cite{resnet} and EfficientNet~\cite{efficientnet}.
